Counterfactual Explanations for Models of Code

Machine learning (ML) models play an increasingly prevalent role in many software engineering tasks. However, because most models are now powered by opaque deep neural networks, it can be difficult for developers to understand why the model came to a certain conclusion and how to act upon the model's prediction. Motivated by this problem, this paper explores counterfactual explanations for models of source code. Such counterfactual explanations constitute minimal changes to the source code under which the model "changes its mind". We integrate counterfactual explanation generation to models of source code in a real-world setting. We describe considerations that impact both the ability to find realistic and plausible counterfactual explanations, as well as the usefulness of such explanation to the user of the model. In a series of experiments we investigate the efficacy of our approach on three different models, each based on a BERT-like architecture operating over source code.

==> background.tex <==
\section{Background \& Related Work}

For explanations in models of code, we focus on local explanation techniques that produce explanations of a specific instance of the input space for a prediction given by the model. Further, given the variety of model families used at Facebook, we focus on model-agnostic techniques. We consider a model to be a learned black-box function $f$ that maps an input $x \in X \subset R^d$ to an output $f(x) \in Y, f : R^d \mapsto Y$. In local explainability, we want to formulate an explanation function $g$ that explains why $f$ predicted $f(x)$ for a particular point $x$.

Several methods have been proposed to provide explanations for model predictions. We can broadly characterize them as white-box (attention- and gradient-based), and perturbation-based mechanisms.

\subsection{White-box Explanation Mechanisms}
Attention-based mechanisms can provide a window into how a model operates. We can extract weights from attention layers and conveniently attach them for each input token~\cite{clark:19, galassi:20, li:16, vashishth:19}. However, recent work has called into question whether using attention weights as feature attribution actually surmounts to an explanation of model behavior, showing that different weights can lead to the same prediction~\cite{jain:19}. Other work has even shown that we can systematically manipulate attention in a network while still retaining the same prediction~\cite{pruthi:20}.

Other work proposed leveraging the dynamics of gradients to diagnose where the model pays the most ``attention". 
One of the recent gradient-based mechanisms for finding local explanations is integrated gradients~\cite{sundararajan:17}, where the idea is to create interpolations of the input and evaluate the model on those interpolated inputs. Unfortunately, unlike image data, code does not lend itself easily to interpolation. For instance, there is no meaningful token to be had by combining embedding of a pad token and a keyword token arithmetically.

\subsection{Perturbation-based Explanation Mechanisms}

Perturbation-based mechanisms remove or replace a subset of features in the input space and track the score differential of the model prediction. The aggregated score difference over many samples is then attributed to features involved in the perturbation. We explored several perturbation-based mechanisms including SHAP with unsatisfactory results. Local surrogate methods, such as LIME~\cite{lime}, generate a new dataset consisting of perturbed samples and the corresponding predictions of the existing model. From our experience, these methods perform poorly because perturbations to source code inputs must adhere to strict semantic guidelines such that the resulting source code retain the structure of a working program. We found that counterfactual explanations, another related concept to find explanations, to be a better fit for finding explanations for models of source code.

There have been several papers that investigate interpretation of models of code through perturbation:
\begin{itemize}
    \item Understanding Neural Code Intelligence Through Program Simplification, FSE'21: Uses delta-debugging to reduce program up until it changes its mind, i.e., produces a “minimal” program that still has the same prediction as the original. The paper dismisses robustness issues for models of source code, Section 7.2 last paragraph: \emph{“For linguistic expressions, input perturbations are usually less obvious: while certain words (such as stop words) may safely be removed without altering the meaning of a sentence, more general changes quickly risk producing very different inputs. Recent input-related methods rely on synonym datasets and swap out similar names to ensure that they generate semantically similar phrases ... Our work shows that, at least for current models and tasks, this is significantly less of a concern in software engineering, where many tokens can be removed with little consequence“}

    % https://arxiv.org/pdf/2106.03353.pdf
    \item Probing Model Signal-Awareness via Prediction-Preserving Input Minimization, FSE'21 
    % https://arxiv.org/pdf/2011.14934.pdf
    \item PyExplainer: Explaining the Predictions of Just-In-Time Defect Models, ASE'21 $\mapsto$ focus on tabular data, not source code perturbation, uses a variation of LIME
    \item Autofocus: Interpreting attention-based neural networks by code perturbation, ASE'19
\end{itemize}


\subsection{Counterfactual Explanations}

Counterfactuals in NLP. Paper links below items as comments.
\begin{itemize}
    \item Polyjuice: Generating Counterfactuals for Explaining, Evaluating, and Improving Models % (https://arxiv.org/pdf/2101.00288.pdf)
    \item Explaining NLP Models via Minimal Contrastive Editing (MICE)
    \item Generate Your Counterfactuals: Towards Controlled Counterfactual Generation for Text % (https://arxiv.org/pdf/2012.04698.pdf)
    \item  Generating Plausible Counterfactual Explanations for Deep Transformers in Financial Text Classification
    \item Generative Counterfactuals for Neural Networks via Attribute-Informed Perturbation: %https://arxiv.org/pdf/2101.06930.pdf
    \item Mask and Infill: Applying Masked Language Model to Sentiment Transfer %(https://arxiv.org/pdf/1908.08039.pdf)
    \item Generative Counterfactuals for Neural Networks via Attribute-Informed Perturbation %(https://arxiv.org/pdf/2101.06930.pdf)
\end{itemize}

\subsection{Robustness and Adversarial Examples}

Mix of adversarial examples of code, robustness, and a few papers investigating the relationship between between robustness and counterfactuals. Paper links below items as comments.

Adv. Examples of Source Code:
\begin{itemize}
    \item Adversarial examples for models of code~\cite{yefet:20}
    \item STRATA: Simple, Gradient-Free Attacks for Models of Code 
    % https://arxiv.org/pdf/2009.13562.pdf
    \item Towards the Unification and Robustness of Perturbation and Gradient Based Explanations: % \url{https://teamcore.seas.harvard.edu/files/teamcore/files/unification_and_robustness_of_perturbation_and_gradient_based_explanations_icml_2021.pdf}
    \item Adversarial Robustness for Code
    % http://proceedings.mlr.press/v119/bielik20a/bielik20a.pdf
    \item Generating adversarial examples for holding robustness of source code processing models, AAAI'20~\cite{zhang:20}
    % https://ojs.aaai.org/index.php/AAAI/article/view/5469/5325
    \item Semantic robustness of models of source code~\cite{semanticrobustness}
    % https://arxiv.org/pdf/2002.03043.pdf
    \item On the generalizability of Neural Program Models with respect to semantic-preserving program transformations
    % https://www.sciencedirect.com/science/article/pii/S0950584921000379
\end{itemize}

Connection Robustness and Counterfactuals
\begin{itemize}
    \item On the Connections between Counterfactual Explanations and Adversarial Examples~\cite{pawelczyk:21}
    % https://arxiv.org/pdf/2106.09992.pdf
    \item Semantics and explanation: why counterfactual explanations produce adversarial examples in deep neural networks
    % https://arxiv.org/pdf/2012.10076.pdf
    \item The Dangers of Post-hoc Interpretability: Unjustified Counterfactual Explanations, IJCAI'19~\cite{laugel:19}
    % https://www.ijcai.org/Proceedings/2019/0388.pdf
    \item The Intriguing Relation Between Counterfactual Explanations and
Adversarial Examples -- quite philosophical, potentially out of scope
    % https://arxiv.org/pdf/2009.05487.pdf
\end{itemize}





==> clipboard/algos.tex <==
\begin{algorithm}[t]
\DontPrintSemicolon
  
  \KwInput{\textbf{Input:} Input program $P$, Model $\mathcal{M}$: $\mathcal{D} \mapsto \{T, F\} \times \mathcal{R}$ returning a classification and a score, iteration count \texttt{ITER}}
  \KwOutput{\textbf{Output}: List of counterfactuals which lead to prediction changes}
  %$\sum_{i=1}^{\infty} := 0$ \tcp*{this is a comment}
  %\tcc{Now this is an if...else conditional loop}
  
  original\_class, \_ = $\mathcal{M}(P)$\\ 
  explanations = []\\
  explore\_heap = \{\}\\
  \For{$p_i \in \mathcal{T}(P)$}{
    $flipped, score, P' = PredictionFlip(P, M, p_i)$\\
    \If{flipped} {
        explanations.add($\langle p_i, P'\rangle$)
    }
    \Else {
        explore\_heap.push($\langle p_i, score \rangle$)
    }
  }
  items = explore\_heap.toList()\\
  
  \For{\_ in \texttt{ITER}} { 
    \tcc{greedy search for \texttt{ITER} iterations}
    best\_token = expore\_heap.pop()\\
    combos = expand\_by\_one(items, best\_token)\\
    \For{combo in combos}{
        \tcc{combo is a set of tokens $\langle p_i,\ldots, p_m \rangle$}
        $flipped, score, P' = PredictionFlip(P, M, combo)$\\  
        \If{flipped} {
            explanations.add($\langle combo, P'\rangle$)
        }
        \Else {
            explore\_heap.push($\langle combo, score \rangle$)
        }        
    }
    return explanations
  }

\caption{GenerateCounterfactualExplanations}
\end{algorithm}

\begin{algorithm}[t]
\DontPrintSemicolon
  
  \KwInput{\textbf{Input:} Input program $P$, Model $\mathcal{M}$, Token or token combination to perturb $\langle p_1, \ldots, p_k \rangle$ where $p_i \in \mathcal{T}(P)$\\}
  \KwOutput{\textbf{Output}: Prediction change (boolean), Score after perturbation, Input after perturbation $P'$}
  \\
    $P' = perturb(P, $\langle p_1, \ldots, p_k \rangle$)$\\
    original\_class, \_ = $\mathcal{M}(P)$\\
    class, score = $\mathcal{M}(P')$\\
    flip = original\_class != class\\
    return $\langle flip, score, P' \rangle$

\caption{PredictionFlip}
\end{algorithm}

==> clipboard/discussion.tex <==
\subsection*{MLM vs. Hand-crafted Perturbation}

What are the nature of code Perturbations produced through MLM?
We identified three distinct categories during the course of our qualitative analysis. Note that the examples we provide in the following are similar to the ones we found in our investigation to be representative to the identified category, but are not actually part of our codebase.
\begin{enumerate}
    \item \emph{Specialized Concept to Generalized Concept:} This is the most common kind of perturbation we have encountered in various different contexts. A very specialized token is replaced with a more generic or generalized version of it. There are several examples of this we found in our sample: In web development replacing a specialized component tag name with a more generic tag name (\texttt{<UIButton>} $\longmapsto$ \texttt{<div>}). Specific class to more generic class in the type hierarchy\\(\texttt{DistributedTask} $\longmapsto$ \texttt{GeneralTask}). And similarly with function calls (\texttt{genNativeRenderTea()} $\longmapsto$ \texttt{gen()}).
    Similar patterns continue in different contexts.
    
    \item \emph{Variable Name/Function Name Correspondence:} Often, when the return value of a function invocation is assigned to a variable, function and variable name tend to have a correspondence. If that was not already the case in the original instance, this kind of perturbation we observed replaces either function or variable name to correspond (e.g., \texttt{prime = is\_prime(x)}).
    \todo{ID: I don't understand this.}
    
    \item \emph{Maximal Contrast:}
    % TODO: This is terrible. I'll refactor later (@JCito)
    Some perturbations, albeit the minority we found in our sample, seemingly follow no pattern. However, they still do achieve their goal in providing what we call a ``maximal contrast" between the original input and the counterfactual.
    \todo{Isn't this a good justification for using MLM in the first place? i.e., it can find useful counterfactuals that are not easy to capture with patterns. This is presented as a bug but seems like a feature :) }
\end{enumerate}

For some downstream tasks, MLM is certainly part of an end-to-end solution to produce counterfactuals in a human-in-the-loop system. For other tasks, where quality of the counterfactuals that MLM provides varies, it is still a good tool for exploration as to why kind of perturbations we can turn into hand-crafted operators to apply in a production setting.

==> findings_old.tex <==
\section{Evaluation}

We show where counterfactuals work well and where their limitations are by performing several experiments.

\subsection{Models and Datasets}
We want to explore 
\begin{itemize}
    \item Method Name Prediction PLBART (open source)
    \item DiffBERT + Screenshot prediction dataset (industry)
\end{itemize}

\subsection{Baselines and Approaches}
\begin{itemize}
    \item Naive Greedy Search (Counterfactual Removal)
    \item SHAP or LIME? \textbf{JC: or none of those because we've already shown they don't work well wrt. robustness}
    \item MaskFilling
    \item Denoising Generative Mask Filling
    \item Attention (Saliency Maps)
    \item Program Simplification (FSE'21)
    %\item $C^2$-EP (Code Counterfactual Explanations Perturbations)
\end{itemize}

\subsection{Sampling and Ground Truth}

To enable quantitative comparison between the different approaches, we need to obtain ground truth labels for what domain experts deem to be explanation attributions. We sample 30 instances from each dataset and let domain experts label which code feature they think is the most appropriate \textbf{JC: why 30? kind of a folklore minimum sample size that we learn in undergrad stats. I have to think about this and re-read the sampling in software engineering guide book).}

\subsection{Experiments and Methodology}

\begin{itemize}
    \item \emph{Quantitative Experiment}: Report accuracy, precision, recall for each approach based on overlap 
    %\item \emph{Controlled User Study / Qualitative Survey}: Let developers (i.e., users of the system) rate explanations and then we compare which one they like better. Retrieve additional qualitative feedback. Do this internally for DiffBERT and also potentially send survey to other people for open source model/dataset. \textbf{Here, we should probably pick 1 baseline to compare to that was closest in quantitative performance?} 
    \item \emph{Performance Experiment}: Compare explanation generation time across techniques and parameters
\end{itemize}

\subsection{Results}
...

\section{Threats to Validity}
....

==> motivation.tex <==
\section{The Need for Model Explanation}

Let us consider learned binary classification model that takes as input a "diff", i.e. a commit (a series of code additions, deletions, and context code lines around the changes) and returns a probability whether the commit will introduce a performance problem~\cite{cito:19, weber:21, deepperf}.

%\begin{listing}
\begin{minted}
[
frame=lines,
framesep=2mm,
baselinestretch=1.2,
bgcolor=LightGray,
fontsize=\footnotesize,
linenos
]{Javascript}
  async function handleTask(taskManager, taskId) {
    const starter = await taskManager.getStarted()
+   const startTime = await taskManager.getTime()
    if(starter.endTime < startTime) {
-     starter.requestNextTask = False
+     starter.requestNextTask = True
+     handleCanceledTask(taskManager, taskId)
    }
+   starter.push(taskId)
+   starter.dispatch()
}

...

+ async function editTask(taskManager, taskId, data) {
+    task = taskManager.find(taskId)
+    task.cancel()
+    handleCanceledTask(taskManager, taskId)
+    task.update(taskId, data)
+    task.resetTime()
+    handleTask(taskId)
+ }
...
    
+ async function handleCanceledTask(taskManager, cancelTaskId) {
+   for(task of taskManager.all()) {
+     if(task.id == cancelTaskId) {
+       taskManager.prune(task)
+     }
+   }
+       
}
\end{minted}
%\caption{Commit labeled as potentially introducing a performance issue by a machine learning model}
%\label{lst:motivation}
%\end{lising}

The code example above represents a larger commit that was labeled as potentially introducing a performance regression by such a machine learning model.
The developer of this commit is confused at first as they are not immediately aware of anything that even has the potential of introducing such an issue.

%\paragraph{\textbf{Scenario 0: No explanation available}:} 

In the current status quo, the developer has to start a complex investigation process that involves hypothesis building, statically inspecting potential culprits, and expensive testing with delta-debugging that involves benchmarks~\cite{baltes:15}. If it then turns out that the machine learning prediction was a false positive, it could lead to frustration well-known from existing experiences when deploying any kind of uncertain program analysis~\cite{tricorder, christakis:16, sadowski:18}.

To avoid unnecessary grievances we introduce our system that generates counterfactual explanations.
We produce a minimally different commit that would \emph{not} be classified as a performance regression.

Let us revisit two scenarios of how our explanations bring value in this situation.

\paragraph{\textbf{Scenario 1: False Positive Explanation}:}

Our explanation attributes the prediction Line 3 in our commit: When changing \texttt{await taskManager.getTime()} to calling a different method \texttt{find}, the classifier changes its mind.
The developer is now guided to investigate the this method invocation. They inspect the \texttt{getTime} method and can verify that there is nothing that can cause a performance regression.
They conclude that the machine learning model must have picked up on a spurious correlation (potentially involving the \texttt{await} keyword indicating an asynchronous call).
The explanation has enabled the developer to understand the inner working of the model and move on quickly, not having wasted time on a false-positive.

\paragraph{\textbf{Scenario 2: True Positive Explanation}:}

Let us consider a case in which the prediction is a true positive. In this case, the explanation points to line 28 in our commit: When changing \texttt{prune(task)} to a different method \texttt{update(task)}, the classifier changes its mind. The developer again is guided in their exploration and this time the inspection reveals that actually the \lstinline{prune} method is indeed the culprit. The developer can now revisit the design of their code contribution.
\\
In both cases, the explanation achieved its goal. It provided guidance to the developer by pointing out similar, but plausible scenarios in which the model changed its mind.

\todo{
    1. Show two different examples for false positive and true positive (instead of the same commit)
    2. show what our method actually does, currently sounds too hypothetical
}


%\begin{itemize}
%    \item Add sketch of input + its explanation
%    \item describe context
%    \item You are confronted with a positive prediction: we think there is a performance problem in this %commit
%    \item You need to decide how to interpret this prediction and define your action space
%    \item Case based reasoning: True Positive, False Positive - how does it to identify either of the cases?
%    \item Here are the questions that you may ask if you are (1) a developer, and (2) model developer %debugging
%\end{itemize}





==> naive_perturbation_study.tex <==
\section{Preliminary Observation: Naive Perturbations expose Robustness Issues}

We explore the efficacy of existing perturbation-based methods and find that rather than providing explanations, they expose model robustness issues.

We applied two naive perturbation-based explanation methods, SEDC and SHAP, to an internal auto complete model based on an LSTM.
We sample N=X instances from a public dataset (ETH dataset?) and apply explanations to it.
We report on the distributions of explanations found with both approaches.
Two authors of this paper qualitatively analyze each of the explanations and label whether an explanation is reasonable or an indication of a robustness issue instead.
    
%, which assign attributions to input features (i.e., source code tokens)
%\item We obtain ground truth attributions for a sample of N in dataset Y hand-labeling instances
%\item We report accuracy, precision, and recall of the methods
%\item For false positive attributions, we qualitatively analyze the input to determine the nature of the false positive label

%X\% of explanations in our sample expose robustness issues.

Initially experimentation showed that simply removing a set of tokens does not lead to satisfying explanations. This phenomenon can be observed both in natural language and source code tasks. Let us have a look at two very unsatisfying explanations for a canonical NLP dataset, IMDBM. When using  naive explanation methods, we were able to see that removing either the tokens ['by', '.'] or ['by', '+'] leads the model to predict differently (without altering the semantics of the input).

In our autocomplete model, we similarly see that removing syntactic tokens leads to a significant change in prediction. Removing \emph{['=', '[']} leads to the model predicting the wrong token and original prediction not even being in the Top-3 predictions any more.

Rather than finding explanations, we have now actually found something akin to adversarial examples known from research in model robustness. Reflecting on this finding, we found that the definition of adversarial examples only differs in one particular aspect: What is a (minimal) set of \emph{imperceptible} changes to a specific input, such that the classification of that input changes?  This has different meaning for different kinds of input spaces. For images, the perturbation should be imperceptible to the human eye. For text, the perturbation often produces synonyms of features~\cite{riberio:18}. For source code, the perturbation could include operations such as alpha renaming~\cite{semanticrobustness}. The goal is testing semantic robustness of the models: would the model predict differently given two semantically equivalent input instances?
